Autonomous System Safety Properties with Multi-Machine Hybrid Event-B

Event-B is a well known methodology for the verified design and development of systems that can be characterised as discrete transition systems. Hybrid Event-B is a conservative extension that interleaves the discrete transitions of Event-B (assumed to be temporally isolated) with episodes of continuously varying state change. While a single Hybrid Event-B machine is sufficient for applications with a single locus of control, it will not do for autonomous systems, which have several loci of control by default. Multi-machine Hybrid Event-B is designed to allow the specification of systems with several loci of control. The formalism is succinctly surveyed, pointing out the subtle semantic issues involved. The multi-machine formalism is then used to specify a relatively simple incident response system, involving a controller, two drones and three responders, working in a partly coordinated and partly independent fashion to manage a putative hazardous scenario.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{Matt Luckcuck and Mengwei Xu (Eds.): \\
Sixth International Workshop on Formal Methods\\
for Autonomous Systems (FMAS 2024)\\
EPTCS 411, 2024, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.411.1}{10.4204/EPTCS.411.1}}
\pdfoutput=1

